Language and Knowledge Representation: A Stratified Approach

The thesis proposes the problem of representation heterogeneity to emphasize the fact that heterogeneity is an intrinsic property of any representation, wherein, different observers encode different representations of the same target reality in a stratified manner using different concepts, language and knowledge (as well as data). The thesis then advances a top-down solution approach to the above stratified problem of representation heterogeneity in terms of several solution components, namely: (i) a representation formalism stratified into concept level, language level, knowledge level and data level to accommodate representation heterogeneity, (ii) a top-down language representation using Universal Knowledge Core (UKC), UKC namespaces and domain languages to tackle the conceptual and language level heterogeneity, (iii) a top-down knowledge representation using the notions of language teleontology and knowledge teleontology to tackle the knowledge level heterogeneity, (iv) the usage and further development of the existing LiveKnowledge catalog for enforcing iterative reuse and sharing of language and knowledge representations, and, (v) the kTelos methodology integrating the solution components above to iteratively generate the language and knowledge representations absolving representation heterogeneity. The thesis also includes proof-of-concepts of the language and knowledge representations developed for two international research projects - DataScientia (data catalogs) and JIDEP (materials modelling). Finally, the thesis concludes with future lines of research.

==> source/readme.tex <==
%
% Author: DISI Department - Technical Staff 
% https://www.disi.unitn.it
%
% License CC BY-SA Attribution-ShareAlike 4.0
% This license lets you remix, tweak, and build upon your work even for commercial purposes,
% as long as they credit you and license their new creations under identical terms.
% 
%
% Last update: May 20, 2024
%

\chapter*{\textit{Suggested thesis structure}}
\markboth{Suggested thesis structure - to be removed}{}
\textit{Chapter to be removed}

\begin{enumerate}
    \item \textbf{Introduction}\\
    This section introduces the problem and provides its positioning in the framework of the main research areas of ICT (telecommunications, computer science, electronics).
    \begin{enumerate}[label*=\arabic*.]
        \item \textbf{The Context}\\
        Describe here the context within which the thesis must be positioned.
        \item \textbf{The Problem}\\
        Here is a short description of the problem.
        \item \textbf{The Solution}\\
        Here is a short description of the solution.
        \item \textbf{Innovative Aspects}\\
        Here is a short description of how the thesis improves the state of the art.
        \item \textbf{Structure of the Thesis}\\
        Here is a short description of the structure of the thesis, possibly section by section.
    \end{enumerate}

    \item \textbf{State of the Art}\\
    Describe here the state of the art of the research of this thesis.
    This part should contain all the relevant publications in the area with the corresponding citations.
    The cited works should be briefly described and critically assessed.
    [Alternatively, the critical reviews could be left to the later chapter “Related work”; this approach could be more suitable for those cases where the results of the thesis – described in chapter 4 – are to be compared in detail with results from other researchers]

    \item \textbf{The Problem}\\
    Describe the problem you have dealt with here.

    \item \textbf{The Proposed Approach} (can be split into several chapters)\\
    One or more chapters should be devoted to describing the proposed approach.

    \item \textbf{Experimental Results}\\
    \textit{(If there is experimental work)}\\
    An experimental results chapter may be necessary to demonstrate the value of the thesis work.

    \item \textbf{Related Work}\\
    One or more chapters should be devoted to a detailed analysis of the related work.
    The content of this section differs from those of the state of the art because the analysis is more detailed here. 
    This chapter must explicitly refer to the contents of the previous chapters (in particular those describing the proposed solution).\\
    (see also chapter 2)

    \item \textbf{Conclusions}\\
    Conclusions should summarize the problem, the solution, and its main innovative features, outlining future work on the topic or application scenarios of the proposed scheme.

\end{enumerate}

\begin{enumerate}[label=\Alph*]
    \item \textbf{Appendix}\\
    \textit{Zero, one or more appendixes.}\\
    The appendix should be used to maintain a record of work that was related and strictly connected to the
    thesis work, but that could be left out from the thesis as a scientific publication.
    For example:
    \begin{itemize}
        \item source code of programs;
        \item laboratory setup and tests configurations;
        \item measurements.
    \end{itemize}
    This information could be published in the form of a dept. tech report or a laboratory internal publication instead of an appendix; these publications should then be cited within the thesis.
\end{enumerate}

\section*{\textit{Generate pdf}}
\textit{Section to be removed}

It is supposed to have
\begin{itemize}
    \item {\texttt main.tex} as main file
    \item \texttt{pdflatex} program
    \item \texttt{bibtex} as bibliography generator
\end{itemize}

To generate pdf, run
\begin{verbatim}
    pdflatex main.tex
    bibtext main
    pdflatex main.tex
    pdflatex main.tex
\end{verbatim}

Finally, rename \texttt{main.pdf} file according to the rule of the school/department.

